On the Powerfulness of Textual Outlier Exposure for Visual OoD Detection

Successful detection of Out-of-Distribution (OoD) data is becoming increasingly important to ensure safe deployment of neural networks. One of the main challenges in OoD detection is that neural networks output overconfident predictions on OoD data, make it difficult to determine OoD-ness of data solely based on their predictions. Outlier exposure addresses this issue by introducing an additional loss that encourages low-confidence predictions on OoD data during training. While outlier exposure has shown promising potential in improving OoD detection performance, all previous studies on outlier exposure have been limited to utilizing visual outliers. Drawing inspiration from the recent advancements in vision-language pre-training, this paper venture out to the uncharted territory of textual outlier exposure. First, we uncover the benefits of using textual outliers by replacing real or virtual outliers in the image-domain with textual equivalents. Then, we propose various ways of generating preferable textual outliers. Our extensive experiments demonstrate that generated textual outliers achieve competitive performance on large-scale OoD and hard OoD benchmarks. Furthermore, we conduct empirical analyses of textual outliers to provide primary criteria for designing advantageous textual outliers: near-distribution, descriptiveness, and inclusion of visual semantics.

==> figs/auxiliary_dataset.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=\textwidth]{raw_figs/auxiliary_all_jmedit.pdf}
  \end{center}
  \caption{Auxiliary dataset analysis. (a) The similarity between the Place and SUN datasets in both the image and text domains.
(b) The similarity between the ID and Places/iNaturalist dataset in the image domain.
(c) The similarity between the ID and iNaturalist dataset in both the image and text domains. See Section~\ref{sec:3.1} for details.} \label{fig:sim}
\end{figure}

==> figs/desc.tex <==
\begin{wrapfigure}{r}{4.5cm}
\begin{center}
\includegraphics[width=0.35\textwidth]{raw_figs/desc.pdf}
  \end{center}
  \caption{An example of class descriptions and CLIP retrieval outputs of outlier prompts based on class descriptions}\label{fig:desc}
\end{wrapfigure}

==> figs/intro.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=0.85\textwidth]{raw_figs/teaser_fig.pdf}
  \end{center}
  \caption{Textual outliers for container ship (working..)}\label{fig:intro}
\end{figure}

==> figs/similarity.tex <==
\begin{wrapfigure}{r}{4.5cm}
\begin{center}
\includegraphics[width=0.35\textwidth]{raw_figs/every_auxiliary_dataset_8.pdf}
  \end{center}
  \caption{Image (orange) and text (blue) }\label{fig:sim}
\end{wrapfigure}

==> figs/vos.tex <==
\begin{wrapfigure}{r}{4.0cm}
\vspace{-10pt}
\centering
\includegraphics[width=4.0cm]{raw_figs/ImageNet10_synthesis_7.pdf}\\[-0.5em]
  \caption{Comparison in outlier synthesis setting}\label{fig:vos}
    \vspace{-13pt}
\end{wrapfigure}

==> tabs/auxdataset/ImageNet10.tex <==
\begin{table}
\setlength{\tabcolsep}{2pt}
  \caption{ImageNet10 vs ImageNet20}
  \label{ImageNet10}
  \small
  \centering
  \renewcommand{\arraystretch}{1.2}
  \begin{tabular}{lccccrcrccrccc}
    \toprule
    \multicolumn{9}{c}{Auxiliary datasets}                   \\
    \cmidrule(r){2-9}
     & \multicolumn{2}{c}{Textures}  &  \multicolumn{2}{c}{Places}  &  \multicolumn{2}{c}{SUN} & \multicolumn{2}{c}{iNaturalist} & ID Acc & \multicolumn{2}{c}{Average} & \multicolumn{2}{c}{stdev} \\
    \midrule
    Outliers & FPR & AUROC & FPR & AUROC & FPR & AUROC & FPR & AUROC & & FPR & AUROC & FPR & AUROC \\
    \midrule
    None &- &-&-&-&-&-&-&-&99.6& 10.70 & 97.86 &- &-\\
    Image & \textbf{3.90} & \textbf{98.79} & \textbf{5.50} & \textbf{98.65} & 10.70 & 97.64 & \textbf{5.50} & 97.80  &  99.6 & \textbf{6.40} & \textbf{98.22} & 2.96 & 0.58 \\
    Text & 9.10 & 98.38 & 9.50 &  98.03 & \textbf{7.80} & \textbf{98.18} & 11.30 & \textbf{97.98} &  \textbf{99.8} & 9.42 & 98.14 & \textbf{1.44} & \textbf{0.17}      \\
    
    \bottomrule
  \end{tabular}
\end{table}





==> tabs/auxdataset/ImageNet100.tex <==
\begin{table}
\setlength{\tabcolsep}{4.5pt}
  \caption{ImageNet100 vs Textures}
  \label{ImageNet100}
  \small
  \centering
  \begin{tabular}{lcccccccccrc}
    \toprule
    \multicolumn{7}{c}{Auxiliary datasets}                   \\
    \cmidrule(r){2-7}
      &  \multicolumn{2}{c}{Places}  &  \multicolumn{2}{c}{SUN} & \multicolumn{2}{c}{iNaturalist} & ID Acc & \multicolumn{2}{c}{Average} & \multicolumn{2}{c}{stdev} \\
    \midrule
    Outliers & FPR & AUROC & FPR & AUROC & FPR & AUROC & & FPR & AUROC & FPR & AUROC \\
    \midrule
    None &- &-&-&-&-&-&  90.6  & 28.56   &  94.89   &&\\
    Image  & 42.89 & 93.22 & 38.65 & 94.06 & \textbf{19.36} & 96.58  &  \textbf{91.2} & 33.63 & 94.62 & 12.54 & 1.74 \\
    Text  & \textbf{20.60} & \textbf{97.26} & \textbf{22.60} & \textbf{97.08} & 22.20 & \textbf{96.94} &  90.0 & \textbf{21.25} & \textbf{97.13} & \textbf{0.86} & \textbf{0.10}      \\
    
    \bottomrule
  \end{tabular}
\end{table}


==> tabs/blip_ablation.tex <==
\begin{wraptable}{r}{5.5cm}
  \caption{caption vs image}
  \label{blip_ablation}
  \centering
  \footnotesize
  \begin{tabular}{lcc}
    \toprule
         & FPR95     & AUROC  \\
    \midrule    
    Image     & 82.88 & 70.70   \\
    Caption     &  59.52 & 85.28   \\
    \bottomrule
  \end{tabular}
\end{wraptable}

==> tabs/finegrained.tex <==
\begin{wraptable}{r}{5.5cm}
\caption{Fine-grained OoD}
  \label{finegrained}
\begin{tabular}{lrrll}
\toprule
& \multicolumn{1}{l}{FPR} & \multicolumn{1}{l}{AUROC} &  &  \\
\midrule
OE & 88.87  & 60.99  &  &  \\
VOS               & 94.79  & 49.25  &  &  \\
\midrule
TOE               & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  \\
~~caption         & 90.71  & 60.70  &  &  \\
~~word            & 89.39  & 62.74  &  &  \\
~~description     & \textbf{87.00} & \textbf{69.14} &  & \\
\bottomrule
\end{tabular}
\end{wraptable}

==> tabs/main_ImageNet100.tex <==
\begin{table}
\setlength{\tabcolsep}{4pt}
  \caption{Comparison of TOE and advanced methods on ImageNet100 dataset.}
  \label{maintable}
  \footnotesize
  \centering
  \begin{tabular}{lccccccccccc}
    \toprule
    \multicolumn{9}{c}{OoD datasets}                   \\
    \cmidrule(r){2-9}
      &  \multicolumn{2}{c}{iNaturalist} & \multicolumn{2}{c}{SUN}  &  \multicolumn{2}{c}{Places} & \multicolumn{2}{c}{Textures} & ID Acc & \multicolumn{2}{c}{Average} \\
    \midrule
    & FPR95 & AUROC & FPR95 & AUROC & FPR95 & AUROC & FPR95 & AUROC && FPR95 & AUROC \\
    \midrule
    OE & 78.31 & 75.23 & 80.10 & 76.55 & 70.41 & 81.78 & 66.38 & 82.04 & 75.51 & 73.80 & 78.90\\
    % CSI  & 75.85 & 82.63 & 90.62 & 47.83 & 94.90 & 44.62 & 85.85 & 87.11 & 74.27 & 86.80 & 65.54 \\
    % SSD+  & 59.60 & 85.54 & 75.62 & 73.80 & 83.60 & 68.11 & 39.40 & 82.40 & \textbf{78.80} & 64.55 & 77.46    \\
    % MixOE & 80.51 & 74.30 & 74.62 & 79.81 & 84.33 & 69.20 & 58.00 & 85.83 & 74.62 & 74.36 & 77.28 \\ 
    VOS  & 94.83 & 57.69 & 98.72 & 38.50 & 87.75 & 65.65 & 70.20 & 83.62 & 74.43 & 87.87 & 61.36 \\ 
    DOE & 55.87 & 85.98 & 80.94 & 76.26 & \textbf{67.84} & \textbf{83.05} & \textbf{34.67} & \textbf{88.90} & 75.50 & 59.83 & 83.54 \\ 
    \midrule
    TOE  & &  &  & & &  &&& &&\\
    ~~none & 84.74 & 74.02 \\
    % ~~image & 62.24 & 84.42 & 69.86 & 79.69 & 89.97 & 68.17 & 95.16 & 54.09 &66.96 & 79.31 & 71.59\\
    ~~desc & 46.25 & 92.07 & 73.85 & 79.63 & 88.71 & 72.87 & 73.62 & 79.77 & 69.50 & 70.60  & 81.08\\
    ~~word & 42.53 & 92.91 & 66.21 & 83.56 & 84.06 & 76.44 & 73.99 & 79.08 & 69.51 & 66.69 & 82.99 \\
    ~~caption & \textbf{38.32} & \textbf{93.27} & \textbf{55.70} & \textbf{86.91} & 71.62 & 81.36 & 72.46 & 79.58 & 71.15 & \textbf{59.52} & \textbf{85.28} \\
    \bottomrule
  \end{tabular}
\end{table}

==> tabs/toe_result.tex <==
\begin{table}
  \caption{Guidelines for Textual Outlier}
  \label{toes}
  \footnotesize
  \centering
  \begin{tabular}{lcccccc}
    \toprule
    
         & Descriptiveness    & Close to boundary  & Jointness & \# of sample & FPR & AUROC\\
    \midrule    
    words    &  &\checkmark & \checkmark & 1393 & 66.69 & 82.99   \\
    descriptions     & \checkmark & \checkmark &  & 5890 & 70.60 & 81.08   \\
    captions &  \checkmark & \checkmark & \checkmark & 4561& \textbf{59.52} & \textbf{85.28}\\ 
    \bottomrule
  \end{tabular}
\end{table}

==> toe_statistics.tex <==
\begin{wraptable}{r}{5.5cm}
\setlength{\tabcolsep}{2.5pt}
  \caption{Textual outlier statistics}
  \label{toe_stats}
  \centering
  \footnotesize
  \begin{tabular}{lccc}
    \toprule
    % \multicolumn{5}{c}{Auxiliary datasets}                   \\
    % \cmidrule(r){2-5}
         &  description  & word & caption  \\
    \midrule    
       & 5890 & 1393 & 4561   \\
    \bottomrule
  \end{tabular}
\end{wraptable}
